Latent Convolutional Models

We present a new latent model of natural images that can be learned on large-scale datasets. The learning process provides a latent embedding for every image in the training dataset, as well as a deep convolutional network that maps the latent space to the image space. After training, the new model provides a strong and universal image prior for a variety of image restoration tasks such as large-hole inpainting, superresolution, and colorization. To model high-resolution natural images, our approach uses latent spaces of very high dimensionality (one to two orders of magnitude higher than previous latent image models). To tackle this high dimensionality, we use latent spaces with a special manifold structure (convolutional manifolds) parameterized by a ConvNet of a certain architecture. In the experiments, we compare the learned latent models with latent models learned by autoencoders, advanced variants of generative adversarial networks, and a strong baseline system using simpler parameterization of the latent space. Our model outperforms the competing approaches over a range of restoration tasks.

==> celebAhalf.tex <==
\section{Half-Image Inpainting}

Image Completions
\begin{figure}[h]
    \centering
    \begin{tabular}{cccccc}
         Distorted Image & LCM & GLO & DIP & WGAN & Original Image\\
         \includegraphics[width=\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image4.png}&
         \includegraphics[width=\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image4.png}&
         \includegraphics[width=\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image4.png}&
         \includegraphics[width=\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image4.png}&
         \includegraphics[width=\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image4.png}&
         \includegraphics[width=\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image4.png}\\
         
    \end{tabular}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

==> celeba_half.tex <==
\begin{figure}[h]
    \centering
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{ccccccc}
         \small{Hole Image} & \small{LCM} & \small{GLO} & \small{DIP} & \small{WGAN} & \small{AE} &\small{Original Image}\\
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image8.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image17.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image18.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image22.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image29.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image43.png}
    \end{tabular}
    \caption{Half-image completion task results on the CelebA dataset ($128 \times 128$ resolution)}
    \label{fig:half-inpaint}
\end{figure}
\begin{figure}[h]
    \centering
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{cccc}
         \small{Distorted Image} & \small{LCM} & \small{GLO} &\small{Original Image}\\
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image2.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image2.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image2.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image2.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image4.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image4.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image4.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image4.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image5.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image5.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image5.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image5.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image6.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image6.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image6.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image6.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image12.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image12.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image12.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image12.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image10.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image10.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image10.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image10.png}\\[-2pt]
    \end{tabular}
    \caption{Image inpainting on CelebA with \(95\%\) of randomly chosen pixels missing.}
    \label{fig:random-inpaint}
\end{figure}


==> celebahq_results.tex <==
\begin{comment}
\begin{table}[h]
 \centering
 \begin{tabular}{@{}ccc@{}}
 \toprule
 \textbf{Model}  & \textbf{Reconstruction Loss} & \textbf{Perceptual Metric} \\ \midrule
 LCM            & 0.0089            & 0.0254            \\ 
 GLO               & 0.0074           & 0.0276               \\ 
 PGAN                & 1.034         & 0.0254                \\ 
 \bottomrule\\
 \end{tabular}
 \caption{Results of Inpainting on the CelebHQ Dataset.}
 \label{tab:Recons-CelebHQ}
\end{table}

\begin{table}[h]
 \centering
 \begin{tabular}{@{}ccc@{}}
 \toprule
 \textbf{Model}  & \textbf{Reconstruction Loss} & \textbf{Perceptual Metric} \\ \midrule
 LCM            & 0.0033           & 0.0228            \\ 
 GLO               & 0.0040           & 0.0236               \\ 
 PGAN                & 0.787         & 0.0275                \\ 
 \bottomrule\\
 \end{tabular}
 \caption{Results of super-resolution on the CelebHQ Dataset.}
 \label{tab:Recons-CelebHQ-supRes}
\end{table}
\end{comment}

\begin{figure}[h]
    %\hspace*{-1.5cm}
    \includegraphics[scale=0.25]{suppmat_figures/Metrics/CelebHQ-Inpaint.png}
    \caption{Results of inpainting on the CelebHQ Dataset}
    \label{fig:met_inpaintHQ}
\end{figure}

\begin{figure}[h]
    %\hspace*{-1.5cm}
    \includegraphics[scale=0.25]{suppmat_figures/Metrics/CelebHQ-Supres.png}
    \caption{Results of super-resolution on the CelebHQ Dataset}
    \label{fig:met_supresHQ}
\end{figure}

\begin{figure}[h!]
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{ccccc}
         \small{Hole Image} & \small{LCM} & \small{GLO} & \small{PGAN}  & \small{Original Image}\\
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Hole_Img/Hole_Image13.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/LCM/Inpainted_Image13.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/GLO/Inpainted_Image13.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/PGAN/Inpainted_Image13.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Org_Img/Org_image13.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Hole_Img/Hole_Image14.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/LCM/Inpainted_Image14.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/GLO/Inpainted_Image14.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/PGAN/Inpainted_Image14.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Org_Img/Org_image14.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Hole_Img/Hole_Image17.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/LCM/Inpainted_Image17.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/GLO/Inpainted_Image17.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/PGAN/Inpainted_Image17.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Org_Img/Org_image17.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Hole_Img/Hole_Image28.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/LCM/Inpainted_Image28.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/GLO/Inpainted_Image28.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/PGAN/Inpainted_Image28.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Org_Img/Org_image28.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Hole_Img/Hole_Image42.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/LCM/Inpainted_Image42.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/GLO/Inpainted_Image42.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/PGAN/Inpainted_Image42.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Org_Img/Org_image42.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Hole_Img/Hole_Image49.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/LCM/Inpainted_Image49.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/GLO/Inpainted_Image49.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/PGAN/Inpainted_Image49.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/Inpainting/Org_Img/Org_image49.png}\\[-2pt]
    \end{tabular}
    \caption{Inpainting on the CelebAHQ dataset.}
    \label{fig:CelebAHQ}
\end{figure}
\begin{figure}[h]
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{ccccc}
         \small{Downsampled Image} & \small{LCM} & \small{GLO} & \small{PGAN}  & \small{Original Image}\\
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Down_Img/Down_Image25.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/LCM/Up_Image25.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/GLO/Up_Image25.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/PGAN/Up_Image25.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Org_Img/Org_image25.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Down_Img/Down_Image36.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/LCM/Up_Image36.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/GLO/Up_Image36.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/PGAN/Up_Image36.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Org_Img/Org_image36.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Down_Img/Down_Image38.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/LCM/Up_Image38.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/GLO/Up_Image38.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/PGAN/Up_Image38.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Org_Img/Org_image38.png}\\[-2pt]
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Down_Img/Down_Image42.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/LCM/Up_Image42.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/GLO/Up_Image42.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/PGAN/Up_Image42.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Org_Img/Org_image42.png}\\[-2pt]
          \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Down_Img/Down_Image46.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/LCM/Up_Image46.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/GLO/Up_Image46.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/PGAN/Up_Image46.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Org_Img/Org_image46.png}\\[-2pt]
          \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Down_Img/Down_Image48.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/LCM/Up_Image48.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/GLO/Up_Image48.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/PGAN/Up_Image48.png}&
         \includegraphics[width=0.20\linewidth]{suppmat_figures/CelebAHQ/SuperRes/Org_Img/Org_image48.png}
         
    \end{tabular}
    \caption{Super-Resolution by a factor of 32 on the CelebAHQ dataset.}
    \label{fig:CelebAHQ-SupRes}
\end{figure}

==> glo_recons.tex <==
\begin{figure}[h!]
    \centering 
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{cccccc}
         \small{Hole Image} & \small{24k (Map)} & \small{8192 (vector)} & \small{4096 (vector)} & \small{2048 (vector)} & \small{Original Image}\\
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image8.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image8.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image8.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image8.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image8.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image8.png}\\[-2pt]
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image10.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image10.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image10.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image10.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image10.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image10.png}\\[-2pt]
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image26.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image26.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image26.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image26.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image26.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image26.png}\\[-2pt]
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image29.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image29.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image29.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image29.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image29.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image29.png}\\[-2pt]
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image30.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image30.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image30.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image30.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image30.png}&
         \includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image30.png}\\[-2pt]
         %\includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image44.png}&
         %\includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image44.png}&
         %\includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image44.png}&
         %\includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image44.png}&
         %\includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image44.png}&
         %\includegraphics[width=0.15\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image44.png}\\[-2pt]
    \end{tabular}
    \caption{Image inpainting using GLO models with latent spaces of different dimension and structure. The column names indicate the dimensionality and the structure of the latent variable used.}
    \label{fig:glo_recons}
\end{figure}

==> suppmat_ICLR.tex <==
% \documentclass{article}

% % if you need to pass options to natbib, use, e.g.:
% % \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading nips_2016
% %
% % to avoid loading the natbib package, add option nonatbib:
% % \usepackage[nonatbib]{nips_2016}

% \usepackage{iclr2019_conference,times}

% % Optional math commands from https://github.com/goodfeli/dlbook_notation.
% %\input{math_commands.tex}
% % \usepackage[final]{nips_2016}

% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{placeins}
% \usepackage{comment}
% \usepackage{courier}
% \usepackage{float}

% \usepackage{subcaption}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{graphicx}
% \newpage
% \title{Latent Convolutional Models (Supplementary)}

% % The \author macro works with any number of authors. There are two
% % commands used to separate the names and addresses of multiple
% % authors: \And and \AND.
% %
% % Using \And between authors leaves it to LaTeX to determine where to
% % break the lines. Using \AND forces a line break at that point. So,
% % if LaTeX puts 3 of 4 authors names on the first line, and the last
% % on the second line, try using \AND instead of \And before the third
% % author name.

% \author{
% %   David S.~Hippocampus\thanks{Use footnote for providing further
% %     information about author (webpage, alternative
% %     address)---\emph{not} for acknowledging funding agencies.} \\
% %   Department of Computer Science\\
% %   Cranberry-Lemon University\\
% %   Pittsburgh, PA 15213 \\
% %   \texttt{hippo@cs.cranberry-lemon.edu} \\
%   %% examples of more authors
%   %% \And
%   %% Coauthor \\
%   %% Affiliation \\
%   %% Address \\
%   %% \texttt{email} \\
%   %% \AND
%   %% Coauthor \\
%   %% Affiliation \\
%   %% Address \\
%   %% \texttt{email} \\
%   %% \And
%   %% Coauthor \\
%   %% Affiliation \\
%   %% Address \\
%   %% \texttt{email} \\
%   %% \And
%   %% Coauthor \\
%   %% Affiliation \\
%   %% Address \\
%   %% \texttt{email} \\
% }



% \newcommand{\fig}[1]{Figure~\ref{fig:#1}}
% \newcommand{\sect}[1]{Section~\ref{sect:#1}}
% \newcommand{\tab}[1]{Table~\ref{tab:#1}}
% \newcommand{\alg}[1]{Algorithm~\ref{alg:#1}}
% \newcommand{\eq}[1]{(\ref{eq:#1})}

% \begin{document}

% \maketitle

% %\input{celebAhalf}


\newpage
\section{Other inpainting tasks}
\label{app:celeba}

Further qualitative comparisons are performed on the CelebA dataset. In \fig{half-inpaint}, we show comparison on the ``extreme'' task of half-image inpainting.  \fig{random-inpaint} gives a comparison for the task of inpainting where 95\% of pixel values are occluded at random. In both cases, the LCM model achieves the best balance of fitting the known evidence and the inpainting quality of known pixels.

\begin{figure}
    \centering
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{ccccccc}
         \small{Hole Image} & \small{LCM} & \small{GLO} & \small{DIP} & \small{WGAN} & \small{AE} &\small{Original Image}\\
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image8.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image17.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image17.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image18.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image18.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image22.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image22.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image29.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Hole_Img/Hole_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/LCM/Inpainted_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/GLO/Inpainted_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/DIP/Inpainted_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/WGAN-GP/Inpainted_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/AE/Inpainted_Image43.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/Half_Inpaintings/Org_Img/Org_image43.png}
    \end{tabular}
    \caption{Half-image completion task results on the CelebA dataset ($128 \times 128$ resolution)}
    \label{fig:half-inpaint}
\end{figure}
\begin{figure}
    \centering
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{cccc}
         \small{Distorted Image} & \small{LCM} & \small{GLO} &\small{Original Image}\\
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image2.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image2.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image2.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image2.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image4.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image4.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image4.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image4.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image5.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image5.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image5.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image5.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image6.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image6.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image6.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image6.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image12.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image12.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image12.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image12.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Hole_Img/Hole_Image10.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/LCM/Inpainted_Image10.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/GLO/Inpainted_Image10.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/RandomMask_Inpainting/Org_Img/Org_image10.png}\\[-2pt]
    \end{tabular}
    \caption{Image inpainting on CelebA with \(95\%\) of randomly chosen pixels missing.}
    \label{fig:random-inpaint}
\end{figure}

\section{Vectorial GLO results}
\label{app:glo}

As a baseline in the main text, we have used the variant of the GLO model \cite{Bojanowski17}, where the latent space is organized as maps leading to ``fully-convolutional'' generator. The latent dimensionality is picked the same as for the the LCM model. Here, we provide evidence that using the original GLO implementation with vectorial-structured latent space, followed by a fully-convolutional layer gives worse results. In particular, we have tried different dimensionality of the latent space (up to 8192, after which we ran out of memory due to the size of the generator). The results for vector-space GLO in comparison with the GLO baseline used in the main text are in \fig{glo_recons} and Table \ref{table:Recons-lossGLO}. The vector based GLO model, despite being trained on latent vector with relatively high dimensionality, clearly underfits. 

\begin{table}
\caption{Training losses of different GLO variants suggesting the underfitting experienced by the vectorial GLO variants.}
 \label{table:Recons-lossGLO}
 \centering
 \begin{tabular}{@{}ccc@{}}
 \toprule
 \textbf{Latent Space Type} & \textbf{Latent Space Dimension} & \textbf{Reconstruction Loss (train)} \\ \midrule
 3D Map            & 24576                  &    0.0113                          \\ 
 Vector                 & 8192                  & 0.0144                              \\ 
 Vector                & 4096                  & 0.0171                             \\ 
 Vector                 & 2048                  & 0.0202                              \\ 
 \bottomrule\\
 \end{tabular}
\end{table}
\begin{figure}
    \centering
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{cccccc}
         \small{Hole Image} & \small{24k (Conv)} & \small{8192 (vec)} & \small{4096 (vec)} & \small{2048 (vec)} & \small{Original Image}\\
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image8.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image8.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image10.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image10.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image10.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image10.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image10.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image10.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image26.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image26.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image26.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image26.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image26.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image26.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image29.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image29.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image30.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image30.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image30.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image30.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image30.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image30.png}\\[-2pt]
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Hole_Img/Hole_Image44.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_Conv/Inpainted_Image44.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_8192/Inpainted_Image44.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_4096/Inpainted_Image44.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/GLO_2048/Inpainted_Image44.png}&
         \includegraphics[width=0.14\linewidth]{suppmat_figures/GLO_Latent/Org_Img/Org_image44.png}\\[-2pt]
    \end{tabular}
    \caption{Image inpainting using GLO models with latent spaces of different dimension and structure. The GLO baseline from the main text achieves the best fit to the known pixels and arguably the best inpaintings of the unknown pixels.}
    \label{fig:glo_recons}
\end{figure}

\section{Latent space prior for GANs}
\label{app:gans}

Most GAN implementations (including ours) use Gaussian prior when sampling in the latent space. In principle, such prior should be imposed during the restoration process (in the form of an additional term penalizing the squared norm of $\textbf{z}$). We however do not impose such prior in the comparisons in the main text, since it makes the underfitting problem of GANs even worse. In \tab{Recons-lossWGAN} we demonstrate that the fitting error for the images from the train set indeed gets worse as the penalty weight is increased. In \fig{wgan_recons}, this effect is demonstrated qualitatively.

\begin{table}
\caption{Reconstruction train losses with different weight penalties using the WGAN-GP.}
 \label{tab:Recons-lossWGAN}
 \centering
 \begin{tabular}{@{}cc@{}}
 \toprule
 \textbf{L2-penalty Weight} & \textbf{Reconstruction Loss} \\ \midrule
 1            & 0.53                  \\ 
 \(1e^{-3}\)                 & 0.3178       \\ 
 \(1e^{-5}\)                & 0.2176        \\
 \(0\)                & 0.1893       \\
 \bottomrule\\
 \end{tabular}
\end{table}

\begin{figure}
    \centering
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{ccccc}
         \small{Original} & \small{0} & \small{1e-5} & \small{1e-3} & \small{1}\\
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/Org_Img/Org_image0.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/0/Inpainted_Image0.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1e-5/Inpainted_Image0.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1e-3/Inpainted_Image0.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1/Inpainted_Image0.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/Org_Img/Org_image8.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/0/Inpainted_Image8.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1e-5/Inpainted_Image8.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1e-3/Inpainted_Image8.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1/Inpainted_Image8.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/Org_Img/Org_image29.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/0/Inpainted_Image29.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1e-5/Inpainted_Image29.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1e-3/Inpainted_Image29.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1/Inpainted_Image29.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/Org_Img/Org_image39.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/0/Inpainted_Image39.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1e-5/Inpainted_Image39.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1e-3/Inpainted_Image39.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/WGAN_Fits/1/Inpainted_Image39.png}\\[-2pt]
    \end{tabular}
    \caption{Image reconstruction using the WGAN-GP with gradually increasing penalties on the norm of the latent representation $\textbf{z}$ as justified by the probabilistic model behind GANs. Increasing the weight of this penalty (shown above) leads to worse underfitting without improving the quality of the reconstruction. Therefore the comparisons in the main text use the variant without such penalty.}
    \label{fig:wgan_recons}
\end{figure}

\section{Architecture details}
\label{app:network}

The architecture details for the components of the LCM model are as follows:
\begin{itemize}
    \item{Generator Network \(g_{\theta}\)}: The generator network \(g_{\theta}\) has an hourglass architecture in all three datasets. In CelebA the map size varies as follows: \(32\times{}32 \rightarrow 4\times4 \rightarrow 128\times128\) and the generator has a total of 38M parameters. In Bedrooms the map size varies as: \(64\times{}64 \rightarrow 4\times4 \rightarrow 256\times256\) and the generator has a total of 30M parameters. In CelebAHQ the map size varies as \(256\times{}256 \rightarrow 32\times32 \rightarrow 1024\times1024\) and the generator has a total of 40M parameters. All the generator networks contain two skip connections within them and have a batch-norm and the LeakyReLU non-linearity after every convolution layer.
    \item{Latent Network \(f_{\phi_{i}}\)}: The latent network used in CelebA128 consists of 4 convolutional layers with no padding. The latent network used in Bedrooms and CelebA-HQ consists of 5 and 7 convolutional layers respectively with no padding.
\end{itemize}
The code of our implementation is available at the project website.

\section{Train/test losses}
\label{app:losses}
For the sake of completeness we provide losses of LCM and GLO models on the training and test set. We additionally provide the loss if the LCM is optimized over the z-space (i.e the output of \(f_{\phi}\)) instead of the parameters of \(f_{\phi}\) (The results shown in row "LCM Z-Space"). In general, the full LCM model has higher loss for train and for test sets, as being more constrained than the other two methods. The additional constraints however allow the LCM model to perform better at image reconstruction tasks.

\begin{table}[h!]
\caption{Reconstruction Loss as measured by the L1-Laploss + MSE on the training and test set. LCM has a higher reconstruction error because while LCM and GLO have the same latent space dimensionality, the LCM additionally imposes the convolutional manifold constrain on the latent space which is absent in GLO. }
\label{tab:recons-loss}
\hspace*{0cm}
\begin{center}
\begin{tabular}{@{}ccc@{}}
\toprule
\textbf{Model Name} & \textbf{Train Set} & \textbf{Test Set} \\ \midrule
\textbf{LCM (Ours)}          & 0.01306                                   & 0.01345                                  \\ \midrule
\textbf{GLO}                 & 0.01007                                 & 0.01033 \\ \midrule
\textbf{LCM Z-Space}         & 0.01205 & 0.01235 
\\ \bottomrule\\
\end{tabular}
\end{center}
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\newpage

\section{More Results on Bedrooms}
\label{app:bedrooms}

In \fig{extrabed}, we provide additional inpainting and superresolution results on the Bedrooms dataset for the compared methods.
\begin{figure}[h!]
    \centering
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{cccccc}
         \small{Distorted} & \small{LCM} & \small{GLO} & \small{DIP} & \small{PGAN} &  \small{Original}\\
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/Hole_Img/Hole_Image16.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/LCM/Inpainted_Image16.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/GLO/Inpainted_Image16.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/DIP/Inpainted_Image16.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/PGAN/Inpainted_Image16.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/Org_Img/Org_image16.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/Hole_Img/Hole_Image17.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/LCM/Inpainted_Image17.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/GLO/Inpainted_Image17.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/DIP/Inpainted_Image17.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/PGAN/Inpainted_Image17.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/Org_Img/Org_image17.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/Hole_Img/Hole_Image23.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/LCM/Inpainted_Image23.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/GLO/Inpainted_Image23.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/DIP/Inpainted_Image23.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/PGAN/Inpainted_Image23.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/Org_Img/Org_image23.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/Hole_Img/Hole_Image24.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/LCM/Inpainted_Image24.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/GLO/Inpainted_Image24.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/DIP/Inpainted_Image24.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/PGAN/Inpainted_Image24.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/Org_Img/Org_image24.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/Hole_Img/Hole_Image33.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/LCM/Inpainted_Image33.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/GLO/Inpainted_Image33.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/DIP/Inpainted_Image33.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/PGAN/Inpainted_Image33.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/Inpainting/Org_Img/Org_image33.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/Down_Img/Down_Image16.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/LCM/Up_Image16.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/GLO/Up_Image16.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/DIP/Up_Image16.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/PGAN/Up_Image16.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/Org_Img/Org_image16.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/Down_Img/Down_Image17.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/LCM/Up_Image17.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/GLO/Up_Image17.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/DIP/Up_Image17.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/PGAN/Up_Image17.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/Org_Img/Org_image17.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/Down_Img/Down_Image23.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/LCM/Up_Image23.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/GLO/Up_Image23.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/DIP/Up_Image23.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/PGAN/Up_Image23.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/Org_Img/Org_image23.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/Down_Img/Down_Image24.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/LCM/Up_Image24.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/GLO/Up_Image24.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/DIP/Up_Image24.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/PGAN/Up_Image24.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/Org_Img/Org_image24.png}\\[-2pt]
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/Down_Img/Down_Image33.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/LCM/Up_Image33.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/GLO/Up_Image33.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/DIP/Up_Image33.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/PGAN/Up_Image33.png}&
         \includegraphics[width=0.12\linewidth]{suppmat_figures/Bedrooms/SuperRes/Org_Img/Org_image33.png}
    \end{tabular}
    \caption{Additional qualitative comparisons on the Bedrooms dataset (see main text for discussion).}
    \label{fig:extrabed}
\end{figure}

%\newpage
% \begin{comment}
% \section{More Results on CelebHQ}
% Here we provide qualitative comparison between LCM and GLO for CelebHQ dataset. \begin{figure}[h]
%     \centering
%     \renewcommand{\tabcolsep}{0.5pt}
%     \begin{tabular}{cccc}
%          \small{Distorted Image} & \small{LCM} & \small{GLO} & \small{Original Image}\\
%          %\includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Hole_Img/Hole_Image6.png}&
%          %\includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/LCM/Inpainted_Image6.png}&
%          %\includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/GLO/Inpainted_Image6.png}&
%          %\includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Org_Img/Org_image6.png}\\[-2.5pt]
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Hole_Img/Hole_Image17.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/LCM/Inpainted_Image17.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/GLO/Inpainted_Image17.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Org_Img/Org_image17.png}\\[-2.5pt]
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Hole_Img/Hole_Image20.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/LCM/Inpainted_Image20.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/GLO/Inpainted_Image20.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Org_Img/Org_image20.png}\\[-2.5pt]
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Hole_Img/Hole_Image26.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/LCM/Inpainted_Image26.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/GLO/Inpainted_Image26.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Org_Img/Org_image26.png}\\[-2.5pt]
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Hole_Img/Hole_Image27.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/LCM/Inpainted_Image27.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/GLO/Inpainted_Image27.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Org_Img/Org_image27.png}\\[-2.5pt]
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Hole_Img/Hole_Image33.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/LCM/Inpainted_Image33.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/GLO/Inpainted_Image33.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Org_Img/Org_image33.png}\\[-2.5pt]
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Hole_Img/Hole_Image40.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/LCM/Inpainted_Image40.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/GLO/Inpainted_Image40.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Org_Img/Org_image40.png}\\[-2.5pt]
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Hole_Img/Hole_Image43.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/LCM/Inpainted_Image43.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/GLO/Inpainted_Image43.png}&
%          \includegraphics[width=0.2\linewidth]{suppmat_figures/CelebHQ/Org_Img/Org_image43.png}\\[-2.5pt]
%     \end{tabular}
% \end{figure}
% \end{comment}




% \end{document}




% \begin{table}[h]
% \centering
% \begin{tabular}{@{}ccc@{}}
% \toprule
% \multicolumn{3}{c}{Generator Architecture for CelebAHQ}                        \\ \midrule
% Layer Number & Layer Type                & Kernel Size                         \\ \midrule
% \multicolumn{3}{c}{\textbf{Input}}                                           \\ \midrule
% 1            & Convolution               & 3x128x4x4, stride=2                 \\
% 2            & Convolution (1)           & 128x256x4x4, stride=2               \\
% 3            & Convolution (2)           & 256x512x4x4, stride=2               \\
% 4            & Convolution               & 512x512x3x3, stride=1, dilation=2   \\
% 5            & Convolution               & 512x1024x3x3, stride=1, dilation=2  \\
% 6            & Convolution               & 1024x1024x3x3, stride=1, dilation=2 \\
% 7            & Convolution               & 1024x1024x3x3, stride=1, dilation=2 \\
% 8            & Convolution               & 1024x512x3x3, stride=1, dilation=2  \\
% 9            & Convolution (2)           & 512x256x3x3, stride=1, dilation=2   \\
% 10           & Convolution Transpose (1) & 768x256x4x4, stride=2               \\
% 11           & Convolution Transpose     & 512x256x4x4, stride=2               \\
% 12           & Convolution Transpose     & 256x128x4x4, stride=2               \\
% 13           & Convolution Transpose     & 128x64x4x4, stride=2                \\
% 14           & Convolution Transpose     & 64x3x4x4, stride=2                  \\ \midrule
% \multicolumn{3}{c}{\textbf{Output}}                                          \\ \bottomrule
% \end{tabular}
% \end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[h]
% \begin{tabular}{@{}ccc@{}}
% \toprule
% \multicolumn{3}{c}{Generator Architecture for CelebA}                          \\ \midrule
% Layer Number & Layer Type                & Kernel Size                         \\ \midrule
% \multicolumn{3}{c}{\textbf{Input}}                                           \\ \midrule
% 1            & Convolution               & 3x256x4x4, stride=2                 \\
% 2            & Convolution (1)           & 256x512x4x4, stride=2               \\
% 3            & Convolution (2)           & 512x1024x4x4, stride=2              \\
% 4            & Convolution               & 1024x1024x3x3, stride=1, dilation=2 \\
% 5            & Convolution               & 1024x1024x3x3, stride=1, dilation=2 \\
% 6            & Convolution (2)           & 1024x1024x3x3, stride=1, dilation=2 \\
% 7            & Convolution Transpose (1) & 2048x512x4x4, stride=2 \\
% 8            & Convolution Transpose     & 1024x512x4x4, stride=2              \\
% 9            & Convolution Transpose     & 512x256x4x4, stride=2               \\
% 10           & Convolution Transpose     & 256x128x4x4, stride=2               \\
% 11           & Bilinear Upsampling       & 2x                                  \\
% 12           & Convolution Transpose     & 128x64x4x4, stride=2                \\
% 13           & Convolution Transpose     & 64x32x4x4, stride=2                 \\
% 14           & Convolution               & 32x3x3x3, stride=1                  \\ \midrule
% \multicolumn{3}{c}{\textbf{Output}}                                          \\ \bottomrule
% \end{tabular}
% \end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[h]
% \begin{tabular}{@{}ccc@{}}
% \toprule
% \multicolumn{3}{c}{Generator Architecture for Bedrooms}                        \\ \midrule
% Layer Number & Layer Type                & Kernel Size                         \\ \midrule
% \multicolumn{3}{c}{\textbf{Input}}                                           \\ \midrule
% 1            & Convolution               & 3x128x4x4, stride=2                 \\
% 2            & Convolution (1)           & 128x256x4x4, stride=2               \\
% 3            & Convolution (2)           & 256x512x4x4, stride=2               \\
% 4            & Convolution               & 512x512x4x4, stride=2               \\
% 5            & Convolution               & 512x1024x3x3, stride=1, dilation=2  \\
% 6            & Convolution (2)           & 1024x1024x3x3, stride=1, dilation=2 \\
% 7            & Convolution Transpose (1) & 1536x512x4x4, stride=2              \\
% 8            & Convolution Transpose     & 1024x512x4x4, stride=2              \\
% 9            & Convolution Transpose     & 512x256x4x4, stride=2               \\
% 10           & Convolution Transpose     & 256x128x4x4, stride=2               \\
% 11           & Convolution Transpose     & 128x64x4x4, stride=2                \\
% 12           & Convolution Transpose     & 64x32x4x4, stride=2                 \\
% 13           & Convolution               & 32x16x3x3, stride=1                 \\
% 14           & Convolution               & 16x3x3x3, stride=1                  \\ \midrule
% \multicolumn{3}{c}{\textbf{Output}}                                          \\ \bottomrule
% \end{tabular}
% \end{table}

